The inverse problem of the Schr\"odinger equation in the plane; A dissection of Bukhgeim's result

The purpose of this licentiate thesis is to present Bukhgeim's result of 2007, which solves the inverse boundary value problem of the Schr\"odinger equation in the plane. The thesis is mainly based on Bukhgeim's paper and Kari Astala's seminar talk, which he gave the 11th and 18th September of 2008 at the University of Helsinki. Section 3 is devoted to the history and past results concerning some related problems: notably the inverse problem of the Schr\"odinger and conductivity equations in different settings. We also describe why some of the past methods do not work in the general case in a plane domain. Section 4 outlines Bukhgeim's result and sketches out the proof. This proof is a streamlined version of the one in Bukhgeim's paper with the stationary phase method based on Kari Astala's presentation. In the following section we prove all the needed lemmas which are combined in section 6 to prove the solvability of the inverse problem. The idea of the proof is simple. Given two Schr\"odinger equations with the same boundary data we get an orthogonality relation for the solutions of the two equations. Then we show the existence of certain oscillating solutions and insert these into the orthogonality relation. Then by a stationary phase argument we see that the two Schr\"odinger equations are the same. In the last section we contemplate an unclear detail in Bukhgeim's paper which Kari Astala pointed out in his seminar talk: without an extra argument Bukhgeim's proof shows the solvability of the inverse problem only for differentiable potentials instead of ones in L^p. But the special oscillating solutions exist even for L^p potentials.

==> cauchy1image.tex <==
\beginpicture
\setcoordinatesystem units <1.12206cm,1.12206cm>
\put {\phantom{.}} at -2.56487 -2.46949
\put {\phantom{.}} at -2.56487 3.01261
\put {\phantom{.}} at 4.56487 -2.46949
\put {\phantom{.}} at 4.56487 3.01261
\setlinear
\setshadesymbol <z,z,z,z> ({\fiverm .})
\setdots<2pt>
\put {$\gamma_1$} at 0.62 0.64
\put {$\gamma_2$} at 3.45 0.69
\put {$\gamma_3$} at 1.3 -1.33
\put {$\gamma_4$} at -1.62 -1.42
\put {$A$} at -1.63 -2.15
\put {$B$} at 3.6 2.54
\put {$C$} at 3.6 -1.27
\put {$D$} at -1.63 -0.77
\putrule from -2.55774 -2.00000 to 4.55774 -2.00000
\putrule from -2.55774 -1.00000 to 4.55774 -1.00000
\putrule from -2.55774 0.00000 to 4.55774 0.00000
\putrule from -2.55774 0.00000 to 4.55774 0.00000
\putrule from -2.55774 1.00000 to 4.55774 1.00000
\putrule from -2.55774 2.00000 to 4.55774 2.00000
%\putrule from -2.55774 3.00000 to 4.55774 3.00000
\putrule from -2.00000 -2.46401 to -2.00000 2.9 %3.00713
\putrule from -1.00000 -2.46401 to -1.00000 2.9 %3.00713
\putrule from 0.00000 -2.46401 to 0.00000 2.9 %3.00713
\putrule from 0.00000 -2.46401 to 0.00000 2.9 %3.00713
\putrule from 1.00000 -2.46401 to 1.00000 2.9 %3.00713
\putrule from 2.00000 -2.46401 to 2.00000 2.9 %3.00713
\putrule from 3.00000 -2.46401 to 3.00000 2.9 %3.00713
\putrule from 4.00000 -2.46401 to 4.00000 2.9 %3.00713
\setsolid
\putrule from 3.20000 -1.00000 to 0.95000 -1.00000
\putrule from 3.20000 -1.00000 to 0.95000 -1.00000
\plot 1.07971 -1.07489 0.95000 -1.00000 /
\plot 1.07971 -0.92511 0.95000 -1.00000 /
\putrule from 0.95000 -1.00000 to -1.30000 -1.00000
\plot -1.30000 -1.80000 0.95000 0.45000 /
\plot -1.30000 -1.80000 0.95000 0.45000 /
\plot 0.80532 0.41124 0.95000 0.45000 /
\plot 0.91124 0.30532 0.95000 0.45000 /
\plot 0.95000 0.45000 3.20000 2.70000 /
\putrule from 3.20000 2.70000 to 3.20000 0.85000
\putrule from 3.20000 2.70000 to 3.20000 0.85000
\plot 3.27489 0.97971 3.20000 0.85000 /
\plot 3.12511 0.97971 3.20000 0.85000 /
\putrule from -1.30000 -1.00000 to -1.30000 -1.40000
\putrule from -1.30000 -1.00000 to -1.30000 -1.40000
\plot -1.22511 -1.27029 -1.30000 -1.40000 /
\plot -1.37489 -1.27029 -1.30000 -1.40000 /
\putrule from -1.30000 -1.40000 to -1.30000 -1.80000
\putrule from 3.20000 0.85000 to 3.20000 -1.00000
\endpicture


==> input_fourierAfterFubini.tex <==
\begin{lemma}
\label{fourierAfterFubini}
If $x, n \in \R$ and $n > 0$, then
\begin{equation}
	\lim_{a\to\infty} \int_{-a}^a e^{-i t x \mp i 2 n t^2}\,dt = \sqrt{\frac{\pi}{n}} e^{\pm i\frac{\phantom{x} x^2}{8n}},
\end{equation}
uniformly over compact set. The choice of the upper or lower symbol in each $\pm$ and $\mp$ must be the same.
\end{lemma}
\begin{proof}
Let $K\subset \R$ be compact and $x\in K$. We begin by transforming the exponent and then making a change of the path of integration. This can be done using Cauchy's theorem.
\begin{equation}
\begin{split}
	\int_{-a}^a &e^{-i t x \mp i 2 n t^2}\,dt = \int_{-a}^a e^{-2n\big( \frac{1\pm i}{\sqrt{2}} t + \frac{x i}{2\sqrt{2}n (1\pm i)}\big)^2 - \frac{x^2}{4n(1\pm i)^2}} \,dt\\
	&= e^{- \frac{x^2}{4n(1\pm i)^2}} \int_{\gamma_1} e^{-2n\eta^2}\,d\sigma(\eta) = e^{\pm i \frac{\phantom{x}x^2}{8n}} \int_{\gamma_1} e^{-2n\eta^2}\,d\sigma(\eta),
\end{split}
\end{equation}
where $\gamma_1$ is the straight line from $A=-\frac{1\pm i}{\sqrt{2}} a + \frac{x i}{2\sqrt{2}n (1\pm i)} = \frac{1\pm i}{\sqrt{2}}\big(-a + \frac{x}{4n}\big)$ to $B=\frac{1\pm i}{\sqrt{2}} a + \frac{x i}{2\sqrt{2}n (1\pm i)} = \frac{1\pm i}{\sqrt{2}}\big(a + \frac{x}{4n}\big)$ in the complex plane. We will show that when $a\longrightarrow\infty$ the integral on $\gamma_1$ gives te same value as on $-\gamma_3$ which is on the real line.\\
\begin{tabular}[c]{ll}
\mbox{\input{cauchy1image.tex}} & 
	\begin{tabular}[c]{l}
		$\displaystyle A = \frac{1\pm i}{\sqrt{2}}\big(-a + \frac{x}{4n}\big)$ \\
		$\displaystyle B = \frac{1\pm i}{\sqrt{2}}\big(a + \frac{x}{4n}\big)$ \\
		$\displaystyle C = \frac{1}{\sqrt{2}}\big(a + \frac{x}{4n}\big)$ \\
		$\displaystyle D = \frac{1}{\sqrt{2}}\big(-a + \frac{x}{4n}\big)$
	\end{tabular}
\end{tabular}

Let's estimate the integrals on $\gamma_2$ and $\gamma_4$. We get
\begin{equation}
\begin{split}
\Big| \int_{\gamma_2} &e^{-2n\eta^2}\,d\sigma(\eta) \Big| = \Big| \int_{\pm \frac{1}{\sqrt{2}}\big(a + \frac{x}{4n}\big)}^0 e^{-2n\big(\frac{1}{\sqrt{2}}(a+\frac{x}{4n}) + it\big)^2}\,dt \Big| \\
&\leq \int_0^{\frac{1}{\sqrt{2}}\big|a + \frac{x}{4n}\big|} e^{-n(a+\frac{x}{4n})^2 + 2n t^2}\,dt \\
&= \frac{1}{\sqrt{2n}} \sqrt{n}\Big|a + \frac{x}{4n}\Big| e^{-n(a+\frac{x}{4n})^2} \int_0^1 e^{n(a+\frac{x}{4n})^2 u^2}\,du \longrightarrow 0,
\end{split}
\end{equation}
when $a \longrightarrow \infty$ by lemma \ref{imagErfAsympt} because $\sqrt{n}\big(a + \frac{x}{4n}\big) \longrightarrow \infty$. This converges uniformly over $x\in K$. Using the same argumentation we also see that $\lim_{a\to\infty} \int_{\gamma_4} e^{-2n\eta^2}\,dm_1(\eta) = 0$ uniformly.

Because the mapping $\eta \mapsto e^{-2n\eta^2}$ is analytic we can use Cauchy's integral theorem. Because $x \in K$ which is compact, we get uniformly
\begin{equation}
\begin{split}
\lim_{a\to\infty} &\int_{-a}^a e^{-i t x \mp i 2 n t^2}\,dt = e^{\pm i \frac{\phantom{x}x^2}{8n}}\lim_{a\to\infty} \int_{\gamma_1} e^{-2n\eta^2}\,d\sigma(\eta) \\
&= e^{\pm i \frac{\phantom{x}x^2}{8n}}\lim_{a\to\infty} \int_{-\gamma_3} e^{-2n\eta^2}\,d\sigma(\eta) = e^{\pm i \frac{\phantom{x}x^2}{8n}}\lim_{a\to\infty} \int_{-a}^a e^{-n(t + \frac{x}{4n})^2} \,dt \\
&=e^{\pm i \frac{\phantom{x}x^2}{8n}} \frac{1}{\sqrt{n}} \int_{-\infty}^\infty e^{-u^2}\,du = \sqrt{\frac{\pi}{n}} e^{\pm i \frac{\phantom{x}x^2}{8n}}.
\end{split}
\end{equation}

\end{proof}


==> input_intProdLim.tex <==
\begin{lemma}
\label{intProdLim}
Let $U \subset \R^n$ be an open set and $m$ a finite measure on it. If $u \in L^p(U,m)$, $(u_i) \subset L^p(U,m)$ and $v \in L^q(U,m)$, $(v_i) \subset L^q(U,m)$, $p, q \geq 2$, such that $\lVert u_i - u \rVert_{L^p(U)} \longrightarrow 0$ and $\lVert v_i - v \rVert_{L^q(U)} \longrightarrow 0$, then
\begin{equation}
	\int_{U} u(x) v(x)\,dm(x) = \lim_{i\to\infty} \int_U u_i(x) v_i(x) \, dm(x).
\end{equation}
\end{lemma}
\begin{proof}
We show that the difference approaches $0$ as $i \longrightarrow \infty$.  By lemma \ref{prodLpqEstimate} we see that
\begin{equation}
\begin{split}
	\Big| \int_U &u(x)v(x) - u_i(x) v_i(x) \,dm(x) \Big| \\
	&\leq \int_U |u(x)v(x) - u(x)v_i(x)| \,dm(x) + \int_U |u(x)v_i(x) - u_i(x)v_i(x)|\,dm(x) \\
	&\leq m(U)^{1-\frac{1}{p}-\frac{1}{q}} \big( \lVert u \rVert_{L^p(U)} \lVert v-v_i \rVert_{L^q(U)} + \lVert u-u_i \rVert_{L^p(U)} \lVert v_i \rVert_{L^q(U)}\\
	&\longrightarrow m(U)^{1-\frac{1}{p}-\frac{1}{q}} \big(\lVert u \rVert_{L^p(U)} \cdot 0 + 0 \cdot \lVert v \rVert_{L^q(U)}\big) = 0,
\end{split}
\end{equation}
when $i \longrightarrow \infty$.
\end{proof}


==> input_prodLpqEstimate.tex <==
\begin{lemma}
\label{prodLpqEstimate}
Let $U \subset \R^n$ be an open set and $m$ a finite measure on it. Then if $f \in L^p(U,m)$ and $g \in L^p(U,m)$, $p,q \geq 2$, we have
\begin{equation}
	\int_U |f(x) g(x)| \,dm(x) \leq m(U)^{1-\frac{1}{p}-\frac{1}{q}} \lVert f \rVert_{L^p(U)} \lVert g \rVert_{L^q(U)}.
\end{equation}
\end{lemma}
\begin{proof}
By H\"older's inequality $\int_U |fg|\,dm(x) \leq \lVert f \rVert_{L^2(U)} \lVert g \rVert_{L^2(U)}$. Again using H\"older we see $\lVert f \rVert_{L^2(U)} = \lVert f^2 \rVert_{L^1(U)}^\frac{1}{2} \leq \big(\int_U dm(x)\big)^{\frac{1}{2} - \frac{1}{p}} \lVert f \rVert_{L^p(U)}$. By doing the same for $g$ we get $\lVert fg \rVert_{L^1(U)} \leq m(U)^{1-\frac{1}{p}-\frac{1}{q}} \lVert f \rVert_{L^p(U)} \lVert g \rVert_{L^q(U)}$.
\end{proof}


==> input_soboCauchyFormula.tex <==
\begin{lemma}[Cauchy formula]
\label{soboCauchy}
Let $p>2$ and $u \in W^{1,p}(\Omega)$. Now
\begin{equation}
\frac{1}{2\pi} \int_{\partial\Omega} \frac{u(z)}{z_0 - z} zd\sigma(z) - \frac{1}{\pi} \int_\Omega \frac{\wbar{\partial}u(z)}{z_0 - z} dm(z) = \begin{cases} u(z_0), & z_0 \in \Omega\\ 0, &z_0 \in \C \setminus \wbar{\Omega} \end{cases}.
\end{equation}
\end{lemma}
\begin{proof}
We will first prove the case $z_0 \in \Omega$. Denote $\Omega_\epsilon = \Omega \setminus B(z_0,\epsilon)$. Note that $\wbar{\partial}u \in L^p(\Omega)$, $p>2$, so $\wbar{\partial}u (z_0 - z)^{-1} \in L^1(\Omega)$. Thus we may use dominated convergence and integration by parts (lemma \ref{soboIntByParts}). Note also that $W^{1,p}(\Omega) \subset C^\alpha(\wbar{\Omega})$, $\alpha = 1-\frac{2}{p}$, so $\Tr u = u_{|\partial\Omega}$ and that $\wbar{\partial} (z_0 - z)^{-1} = 0$ in $\Omega_\epsilon$. Thus
\begin{equation}
\begin{split}
\frac{1}{\pi}& \int_\Omega \frac{\wbar{\partial} u (z)}{z_0 - z} dm(z) = \lim_{\epsilon\to 0} \frac{1}{\pi} \int_{\Omega_\epsilon} \frac{\wbar{\partial} u (z)}{z_0 - z} dm(z)\\
&= \lim_{\epsilon\to 0} \frac{1}{\pi} \Big( \int_{\partial\Omega} \frac{u(z)}{z_0 - z} \frac{z}{2}d\sigma(z) + \int_{S(z_0,\epsilon)} \frac{u(z)}{z_0 - z} \frac{z-z_0}{2\epsilon} d\sigma(z) \Big)\\
&=\frac{1}{2\pi} \int_{\partial\Omega} \frac{u(z)}{z_0 - z} zd\sigma(z) - u(z_0) - \lim_{\epsilon\to 0} \frac{1}{2\pi\epsilon} \int_{S(z_0,\epsilon)} \hspace{-0.8cm}\big( u(z) - u(z_0) \big) d\sigma(z).
\end{split}
\end{equation}
The last term tends to zero because $|u(z) - u(z_0)| \leq \lVert u \rVert_\alpha |z-z_0|^\alpha = \lVert u \rVert_\alpha \epsilon^\alpha$ in the circle $S(z_0,\epsilon)$. If $z_0 \in \C \setminus \wbar{\Omega}$ we get directly $\int_\Omega \frac{\wbar{\partial} u (z)}{z_0 - z} dm(z) =  \int_{\partial\Omega} \frac{u(z)}{z_0 - z} zd\sigma(z)$ because $(z_0 - z)^{-1} \in W^{1,\infty}(\Omega)$.
\end{proof}
